Modeling Choice via Self-Attention

Models of choice are a fundamental input to many now-canonical optimization problems in the field of Operations Management, including assortment, inventory, and price optimization. Naturally, accurate estimation of these models from data is a critical step in the application of these optimization problems in practice. Concurrently, recent advancements in deep learning have sparked interest in integrating these techniques into choice modeling. However, there is a noticeable research gap at the intersection of deep learning and choice modeling, particularly with both theoretical and empirical foundations. Thus motivated, we first propose a choice model that is the first to successfully (both theoretically and practically) leverage a modern neural network architectural concept (self-attention). Theoretically, we show that our attention-based choice model is a low-rank generalization of the Halo Multinomial Logit (Halo-MNL) model. We prove that whereas the Halo-MNL requires $\Omega(m^2)$ data samples to estimate, where $m$ is the number of products, our model supports a natural nonconvex estimator (in particular, that which a standard neural network implementation would apply) which admits a near-optimal stationary point with $O(m)$ samples. Additionally, we establish the first realistic-scale benchmark for choice model estimation on real data, conducting the most extensive evaluation of existing models to date, thereby highlighting our model's superior performance.

==> theorems/thm_low_rank_is_self_attention.tex <==

\begin{theoremEnd}[category=lowrankattention]{proposition}
\label{prop:LowRank-Attention}
    The Low-Rank Halo MNL choice model can be represented as a neural network with a single self-attention head.
\end{theoremEnd}
\begin{proofsketch}
Consider the decomposition in Eq.~\ref{eqn:LowRankHalo}, and compare it to the standard self-attention mechanism outlined in Algorithm 1. In the nomenclature of attention, the matrices $U$ and $V$ encode the $r$-dimensional  {\em queries} and {\em keys} of the $m$  products (when taken to be one-hot encoded). Finally, the {\em values} of the products are simply formed by the canonical basis in $\mathbb{R}^m$.
\end{proofsketch}
\begin{proofEnd}
Recall that the Low-Rank Halo MNL is encoded by $H = \mathrm{diag}(\alpha) + UV^\top$ for $\alpha \in \mathbb{R}^m$ and $U,V \in \mathbb{R}^{m \times r}$. It takes as input an assortment $a \in \{0,1\}^m$, and outputs choice probabilities $p(a) \in \Delta^{m-1}$ according to:
\[ p(a)_i = \frac{a_i \exp(Ha)_i}{a^\top \exp(Ha)},  \]
or equivalently, if the assortments are encoded as $a \in \{0,e\}^m$, then 
\[ p(a) = \mathrm{softmax}(e\log(a) \circ (Ha)).\]

Now consider a neural network with three layers:
\begin{enumerate}
\item {\bf Input:} The input layer consists of $m$ nodes. Note that this is essentially just a tokenization of the products, and any assortment $a \in \{0,1\}^m$ can be input.
\item {\bf Self-attention:} A single self-attention head will compute so-called queries $Q \in \mathbb{R}^{m \times d}$ and keys $K \in \mathbb{R}^{m \times d}$ for some $d \in [m]$. In this case, take $d = r$, and let $Q = U$, and $K = \sqrt{r}V$. The self-attention layer will also compute values $Y \in \mathbb{R}^{m \times d}$ for some $d \in [m]$. In this case, take $d = m$, and let $Y = I$, the identity matrix. The result of this layer, after feeding through an assortment $a$ from the input layer, is $m$ outputs of the form $\frac{QK^\top Va}{\sqrt{r}}$, which is equal to $UV^\top a$.\footnote{Note that there is often a softmax applied to $QK^\top$. We omit this here.}
\item {\bf Output:} The output layer consists of $m$ nodes, and is gotten by taking the softmax of the output of the self-attention head, along with single edges from the input layer with logarithmic activation. Setting the weights on the single edges to be $\exp(\alpha)$, the output is a softmax applied to $e\log(a) \circ (Ha)$ as was needed.
\end{enumerate}
\end{proofEnd}
    

